Quantum symmetries of Cayley graphs of abelian groups

We study Cayley graphs of abelian groups from the perspective of quantum symmetries. We develop a general strategy for determining the quantum automorphism groups of such graphs. Applying this procedure, we find the quantum symmetries of the halved cube graph, the folded cube graph and the Hamming graphs.

==> partmac.tex <==
%%Macro package for typeseting set partitions
%%Daniel Gromada 2019--2020
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%First, also as an example, we define shortcuts for some short partitions using word representation.

%%%Partitions with lower points only

%%k=1

\def\La{\LPartition{0.6:1}{}}

%%k=2

\def\Laa{\LPartition{}{0.6:1,2}}
\def\Lab{\LPartition{0.6:1,2}{}}

%k=3

\def\Laaa{\LPartition{}{0.6:1,2,3}}
\def\Laab{\LPartition{0.6:3}{0.6:1,2}}
\def\Laba{\LPartition{0.4:2}{0.8:1,3}}
\def\Labb{\LPartition{0.6:1}{0.6:2,3}}
\def\Labc{\LPartition{0.6:1,2,3}{}}

%k=4


\def\Laaaa{\LPartition{}{0.6:1,2,3,4}}
\def\Laaab{\LPartition{0.6:4}{0.6:1,2,3}}
\def\Laaba{\LPartition{0.4:3}{0.8:1,2,4}}
\def\Labaa{\LPartition{0.4:2}{0.8:1,3,4}}
\def\Labbb{\LPartition{0.6:1}{0.6:2,3,4}}
\def\Laabb{\LPartition{}{0.6:1,2;0.6:3,4}}
\def\Labba{\LPartition{}{0.8:1,4;0.4:2,3}}
\def\Labab{\LPartition{}{0.8:2,4;0.4:1,3}}
\def\Laabc{\LPartition{0.6:3,4}{0.6:1,2}}
\def\Labac{\LPartition{0.4:2,4}{0.8:1,3}}
\def\Labca{\LPartition{0.4:2,3}{0.8:1,4}}
\def\Labbc{\LPartition{0.6:1,4}{0.6:2,3}}
\def\Labcb{\LPartition{0.4:1,3}{0.8:2,4}}
\def\Labcc{\LPartition{0.6:1,2}{0.6:3,4}}
\def\Labcd{\LPartition{0.6:1,2,3,4}{}}

%%%Partitions with upper points only

%%k=1

\def\Ua{\UPartition{0.4:1}{}}

%%k=2

\def\Uaa{\UPartition{}{0.4:1,2}}
\def\Uab{\UPartition{0.4:1,2}{}}

%k=3

\def\Uaaa{\UPartition{}{0.5:1,2,3}}
\def\Uaab{\UPartition{0.4:3}{0.4:1,2}}
\def\Uaba{\UPartition{0.6:2}{0.2:1,3}}
\def\Uabb{\UPartition{0.4:1}{0.4:2,3}}
\def\Uabc{\UPartition{0.4:1,2,3}{}}

%k=4

\def\Uaaaa{\UPartition{}{0.4:1,2,3,4}}
\def\Uaaab{\UPartition{0.4:4}{0.4:1,2,3}}
\def\Uaaba{\UPartition{0.6:3}{0.2:1,2,4}}
\def\Uabaa{\UPartition{0.6:2}{0.2:1,3,4}}
\def\Uabbb{\UPartition{0.4:1}{0.4:2,3,4}}
\def\Uaabb{\UPartition{}{0.4:1,2;0.4:3,4}}
\def\Uabba{\UPartition{}{0.2:1,4;0.6:2,3}}
\def\Uabab{\UPartition{}{0.2:2,4;0.6:1,3}}
\def\Uaabc{\UPartition{0.4:3,4}{0.4:1,2}}
\def\Uabac{\UPartition{0.6:2,4}{0.2:1,3}}
\def\Uabca{\UPartition{0.6:2,3}{0.2:1,4}}
\def\Uabbc{\UPartition{0.4:1,4}{0.4:2,3}}
\def\Uabcb{\UPartition{0.6:1,3}{0.2:2,4}}
\def\Uabcc{\UPartition{0.4:1,2}{0.4:3,4}}
\def\Uabcd{\UPartition{0.4:1,2,3,4}{}}

%%%Partitions with same amount of upper and lower points

%%k=1, l=1

\def\Paa{\Partition{
\Pline (1,0) (1,1)
}}

\def\Pab{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
}}

%k=4

\def\Paaaa{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
\Pline (1.5,0.3) (1.5,0.7)
}}
\def\Paaab{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:2
\Pline (1,0) (1,0.7)
}}
\def\Paaba{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:1
\Pline (2,0) (2,0.7)
}}
\def\Pabaa{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1
\Pline (2,0.3) (2,1)
}}
\def\Pabbb{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:2
\Pline (1,0.3) (1,1)
}}
\def\Paabb{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabba{\Partition{
\Pline (1,0) (1,1)
\Pline (2,0) (2,1)
}}
\def\Pabab{\Partition{
\Pline (1,0) (2, 1)
\Pline (1,1) (2, 0)
}}
\def\Paabc{\Partition{
\Psingletons 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabcc{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}
\def\Pabac{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:1
\Pline (1,0) (2,1)
}}
\def\Pabcb{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:2
\Pline (2,0) (1,1)
}}
\def\Pabca{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
\Pline (2,0) (2,1)
}}
\def\Pabbc{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:2
\Pline (1,0) (1,1)
}}
\def\Pabcd{\Partition{
\Psingletons 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}

%k=6

\def\Pabcabc{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
}}
\def\Pabcabd{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:3
\Psingletons 1to0.7:1
}}
\def\Pabcadc{\Partition{
\Pline (1,0) (3, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:2
\Psingletons 1to0.8:2
}}
\def\Pabcdbc{\Partition{
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.3:1
\Psingletons 1to0.7:3
}}
\def\Pabcade{\Partition{
\Pline (1,0) (3, 1)
\Psingletons 0to0.2:2,3
\Psingletons 1to0.8:1,2
}}
\def\Pabcdec{\Partition{
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:1,2
\Psingletons 1to0.8:2,3
}}
\def\Pabcdbe{\Partition{
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:1,3
\Psingletons 1to0.7:1,3
}}
\def\Pabcdef{\Partition{
\Psingletons 0to0.3:1,2,3
\Psingletons 1to0.7:1,2,3
}}

\def\Paabaab{\Partition{
\Pblock 1to0.75:2,3
\Pblock 0to0.25:1,2
\Pline (1.5,0.25)(2.5,0.75)
\Pline (3,0)(1,1)
}}

%%%Some aliases

%\def\singleton{{\mathord{\uparrow}}}
%\def\upsingleton{{\mathord{\downarrow}}}
\def\singleton{\LPartition{\Ps1:1}{}}
\def\upsingleton{\UPartition{\Ps0:1}{}}
\let\pairpart=\Laa
\let\uppairpart=\Uaa
\let\fourpart=\Laaaa
\let\idpart=\Paa
\let\disconnecterpart=\Pab
\let\connecterpart=\Paaaa
\let\crosspart=\Pabab
\let\positionerpart=\Pabcb
\let\halflibpart=\Pabcabc


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%The macros

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}
\def\fihere#1\fi{\fi#1}

%definition of the \Partition command
\def\Partition#1{\def\Ptmp{#1}%
\futurelet\nextchar\PartitionB
}

\def\BigPartition#1{\def\Ptmp{#1}%
\futurelet\nextchar\BigPartitionB
}

\def\PartitionD{%
\thinspace\textchoice
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.175em}{0.55em}{0.7em}{\Ptmp}}
{\PartitionA{0.125em}{0.4em}{0.5em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}%
\thinspace%
}

\def\BigPartitionD{%
\thinspace\textchoice
{\PartitionA{1em}{0.9em}{2.5em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}
{\PartitionA{0.25em}{0.5em}{1em}{\Ptmp}}
{\PartitionA{0.20em}{0.4em}{0.8em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}%
\thinspace
}

\newcount\tmpx
\newcount\tmpy
\def\PartitionB{\if[\nextchar\let\next=\PartitionC\else\let\next=\PartitionD\fi\next}
\def\BigPartitionB{\if[\nextchar\let\next=\BigPartitionC\else\let\next=\BigPartitionD\fi\next}
\def\PartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\PartitionD}
\def\BigPartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\BigPartitionD}

\def\Ppointlist#1{\advance\tmpx by 1\if#1]\else
	\csname P#1\endcsname(\the\tmpx,\the\tmpy)
	\fihere\Ppointlist\fi}

\def\Pwidth{0.05}

\def\Phook{}

\def\PartitionA#1#2#3#4{%
\pgfpicture
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Pwidth em}
\Phook
#4
\endpgfpicture
}

%\Pline, \Psingletons, \Pblock, \Ptext,...

\def\Pline(#1,#2)#3(#4,#5){
\pgfpathmoveto{\pgfpointxy{#1}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#5}}
\pgfusepath{stroke}
}

\def\Psingletons #1to#2:#3 {\PsingletonsA{#1}{#2}#3,,}
\def\PsingletonsA#1#2#3,{\ifx,#3,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfusepath{stroke}
\fihere\PsingletonsA{#1}{#2}\fi}

\def\Pblock #1to#2:#3 {\PblockA{#1}{#2}#3,,
\pgfusepath{stroke}
}
\def\PblockA#1#2#3,#4,{\ifx,#4,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#1}}
\fihere\PblockA{#1}{#2}#4,\fi}

\def\Ptext(#1,#2)#3{%
\pgftext[at={\pgfpointxy{#1}{#2}}]{#3}
}

%\LPartition,\Upartition

\def\LPartition#1#2{\Partition{
\LPartitionB#2;;
\LPartitionA#1;;
}}

\def\LPartitionA#1;{\ifx;#1;\else
\Lsingletons #1 
\fihere\LPartitionA\fi}

\def\LPartitionB#1;{\ifx;#1;\else
\Pblock 0to#1 
\fihere\LPartitionB\fi}

\def\UPartition#1#2{\Partition{
\UPartitionB#2;;
\UPartitionA#1;;
}}

\def\UPartitionA#1;{\ifx;#1;\else
\Usingletons #1 
\fihere\UPartitionA\fi}

\def\UPartitionB#1;{\ifx;#1;\else
\Pblock 1to#1 
\fihere\UPartitionB\fi}

\def\Lsingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint0 #1#2 \else\Psingletons 0to#1#2 \fi
}
\def\Usingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint1 #1#2 \else\Psingletons 1to#1#2 \fi
}

%colors

\def\Pcolw{0.1}

\expandafter\def\csname P/\endcsname{\advance\tmpy by1 \tmpx=0}
\expandafter\def\csname P0\endcsname{}

\def\Pw (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
}

\def\Pb (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
}

\def\Ps#1(#2,#3){
	\pgfsetarrowsend{to}
	\pgfpathmoveto{\pgfpointxy{#2}{#3}}
	\pgfpathlineto{\pgfpointxy{#2}{#1}}
	\pgfusepath{stroke}
	\pgftransformreset
	\pgfsetarrowsend{}
}

\def\Pq (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\PQ (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\Lt (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\Ut (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\LT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}
\def\UT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}

\def\Ppoint #1 #2:#3 {\PpointA{#1}{#2}#3,,}
\def\PpointA#1#2#3,{\ifx,#3,\else #2(#3,#1)\fihere\PpointA{#1}{#2}\fi}

\def\coldefA #1 #2{\kern0.1ex\vcenter{\hbox{\def\Pcolw{#1}\pgfpicture#2(0,0)\endpgfpicture}}\kern0.1ex}

\def\coldef#1#2{\def#1{{\textchoice
{\coldefA 0.15 #2}{\coldefA 0.15 #2}{\coldefA 0.1 #2}{\coldefA 0.08 #2}{$\coldefA 0.15 #2$}}}}

\coldef\bcol\Pb
\coldef\wcol\Pw
\coldef\qcol\Pq
\coldef\Qcol\PQ
\coldef\tcol\Lt
\coldef\Tcol\LT

\def\singext{\LPartition{\Lt:1}{}}
\def\upsingext{\UPartition{\Ut:1}{}}
\def\idext{
	\Partition{
	\Lt (1,0)
	\Ut (1,1)
	}}
\def\positionerext{
	\Partition{
	\Lt (1,0)
	\Ut (2,1)
	\Pline(2,0)(1,1)
	}}
\def\globcolext{
	\Partition{
	\Lt (1,0)
	\Ut (3,1)
	\Pline(2,0)(1,1)
	\Pline(3,0)(2,1)
	}}

